Uniformly accurate oscillatory integrators for the Klein-Gordon-Zakharov system from low- to high-plasma frequency regimes

We present a novel class of oscillatory integrators for the Klein-Gordon-Zakharov system which are uniformly accurate with respect to the plasma frequency $c$. Convergence holds from the slowly-varying low-plasma up to the highly oscillatory high-plasma frequency regimes without any step size restriction and, especially, uniformly in $c$. The introduced schemes are moreover asymptotic consistent and approximates the solutions of the corresponding Zakharov limit system in the high-plasma frequency limit ($c \to \infty$). We in particular present the construction of the first- and second-order uniformly accurate oscillatory integrators and establish rigorous, uniform error estimates. Numerical experiments underline our theoretical convergence results.

==> figure1.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.00000,0.17241}%
\definecolor{mycolor2}{rgb}{1.00000,0.10345,0.72414}%
\definecolor{mycolor3}{rgb}{1.00000,0.82759,0.00000}%
\definecolor{mycolor4}{rgb}{0.00000,0.34483,0.00000}%
\definecolor{mycolor5}{rgb}{0.51724,0.51724,1.00000}%
\definecolor{mycolor6}{rgb}{0.62069,0.31034,0.27586}%
\definecolor{mycolor7}{rgb}{0.92900,0.69400,0.12500}%
%
\begin{tikzpicture}

\begin{axis}[%
width=2.0in,
height=2.5in,
at={(0.0in,0.0in)},
scale only axis,
xmode=log,
xmin=0.0001220703125,
xmax=0.5,
xminorticks=true,
xlabel style={font=\bfseries},
xlabel={$\tau$},
ymode=log,
ymin=1e-6,
ymax=0.9,
yminorticks=true,
xtick={1e-1, 1e-2, 1e-3, 1e-4},
ytick={1e-1, 1e-3, 1e-4, 1e-5, 1e-6},
ylabel style={font=\normalsize},
ylabel={$\text{Error in z}$},
axis background/.style={fill=white},
legend style={yshift=-0.15cm,xshift=0.1cm,nodes={scale=0.7, transform shape},legend cell align=left,align=left,draw=white!10!black,legend pos=south east}
]
\addplot [color=blue,solid,line width=2.0pt,mark=o,mark options={solid}]
  table[row sep=crcr]{%
0.5	0.055586532849719\\
0.25	0.0302184945538502\\
0.125	0.0114041066851084\\
0.0625	0.00549552730044718\\
0.03125	0.00291689193335499\\
0.015625	0.00152205228614517\\
0.0078125	0.00077736747890973\\
0.00390625	0.000390764257890963\\
0.001953125	0.000193588694460023\\
0.0009765625	9.39935830235904e-05\\
0.00048828125	4.39393287630912e-05\\
0.000244140625	1.88474182458886e-05\\
0.0001220703125	6.28519105127057e-06\\
};
\addlegendentry{$c$ = 1};

\addplot [color=red,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.0405949868371809\\
0.25	0.0276991921488574\\
0.125	0.0145195529097185\\
0.0625	0.00749113351882388\\
0.03125	0.00644591290929173\\
0.015625	0.00286872912882958\\
0.0078125	0.00218644954628817\\
0.00390625	0.00126745389271027\\
0.001953125	0.000669986083834923\\
0.0009765625	0.000333382508532788\\
0.00048828125	0.000157636210380704\\
0.000244140625	6.79893846547049e-05\\
0.0001220703125	2.2734669135031e-05\\
};
\addlegendentry{$c$ = 10};

\addplot [color=green,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.057749585080492\\
0.25	0.0451347075134446\\
0.125	0.0244582643279609\\
0.0625	0.0118310846374097\\
0.03125	0.00567461033860597\\
0.015625	0.00275967336690062\\
0.0078125	0.001450914730349\\
0.00390625	0.000698001874463238\\
0.001953125	0.000343455478084603\\
0.0009765625	0.000219862594159145\\
0.00048828125	0.000123406541196853\\
0.000244140625	6.51725448382259e-05\\
0.0001220703125	1.322362114743e-05\\
};
\addlegendentry{$c$ = 100};

\addplot [color=mycolor3,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.033886033399357\\
0.25	0.0377779299951301\\
0.125	0.0192799336222326\\
0.0625	0.0105138600915772\\
0.03125	0.00575092856179256\\
0.015625	0.00283440548298271\\
0.0078125	0.00140632374413447\\
0.00390625	0.000691883931390366\\
0.001953125	0.000343350909001317\\
0.0009765625	0.000165888814790438\\
0.00048828125	7.7514669997982e-05\\
0.000244140625	3.3335336366041e-05\\
0.0001220703125	1.11862572923234e-05\\
};
\addlegendentry{$c$ = 1000};

\addplot [color=mycolor4,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.0724476127627824\\
0.25	0.0430154566458451\\
0.125	0.0191428986032965\\
0.0625	0.00937051221102821\\
0.03125	0.00599191245102996\\
0.015625	0.00290944842299778\\
0.0078125	0.00142745312346152\\
0.00390625	0.000702581967810119\\
0.001953125	0.000344334021586022\\
0.0009765625	0.000166278934454716\\
0.00048828125	7.75150150765093e-05\\
0.000244140625	3.32185704347014e-05\\
0.0001220703125	1.10699041835372e-05\\
};
\addlegendentry{$c$ = 10000};

\addplot [color=black,dashed,line width=4.0pt]
  table[row sep=crcr]{%
0.5	0.5\\
0.25	0.25\\
0.125	0.125\\
0.0625	0.0625\\
0.03125	0.03125\\
0.015625	0.015625\\
0.0078125	0.0078125\\
0.00390625	0.00390625\\
0.001953125	0.001953125\\
0.0009765625	0.0009765625\\
0.00048828125	0.00048828125\\
0.000244140625	0.000244140625\\
0.0001220703125	0.0001220703125\\
6.103515625e-05	6.103515625e-05\\
3.0517578125e-05	3.0517578125e-05\\
};
\addlegendentry{$\mathcal{O}(\tau)$};

\end{axis}

\begin{axis}[%
width=2.0in,
height=2.5in,
at={(3.0in,0.0in)},
scale only axis,
xmode=log,
xmin=0.0001220703125,
xmax=0.5,
xminorticks=true,
xlabel style={font=\bfseries},
xlabel={$\tau$},
ymode=log,
ymin=1e-6,
ymax=0.9,
yminorticks=true,
xtick={1e-1, 1e-2, 1e-3, 1e-4},
ytick={1e-1, 1e-3, 1e-4, 1e-5, 1e-6},
ylabel style={font=\normalsize},
ylabel={$\text{Error in n}$},
axis background/.style={fill=white},
legend style={yshift=-0.15cm,xshift=0.1cm,nodes={scale=0.7, transform shape},legend cell align=left,align=left,draw=white!10!black,legend pos=south east}
]
\addplot [color=blue,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.676486292235307\\
0.25	0.297250067157146\\
0.125	0.0838030102284134\\
0.0625	0.0221634410753464\\
0.03125	0.00607799576009037\\
0.015625	0.00180226425110685\\
0.0078125	0.000628766074286798\\
0.00390625	0.000259820097101336\\
0.001953125	0.000118251956673363\\
0.0009765625	5.54046878194233e-05\\
0.00048828125	2.54984309292628e-05\\
0.000244140625	1.08588123716483e-05\\
0.0001220703125	3.60872225568945e-06\\
};
\addlegendentry{$c$ = 1};

\addplot [color=red,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.675727109539905\\
0.25	0.297102189953057\\
0.125	0.0823252573502638\\
0.0625	0.0206792674447262\\
0.03125	0.00506701668564554\\
0.015625	0.0014411828559432\\
0.0078125	0.000523160654445462\\
0.00390625	0.000234051122308833\\
0.001953125	0.000111733198731171\\
0.0009765625	5.35615879389074e-05\\
0.00048828125	2.49136441282593e-05\\
0.000244140625	1.06635388056017e-05\\
0.0001220703125	3.55253656157172e-06\\
};
\addlegendentry{$c$ = 10};

\addplot [color=green,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.675755913057\\
0.25	0.297224369103591\\
0.125	0.0825582419832529\\
0.0625	0.0208445960414273\\
0.03125	0.00525945405303095\\
0.015625	0.00151638558077684\\
0.0078125	0.000556521393103677\\
0.00390625	0.00024566425292134\\
0.001953125	0.000116480987311607\\
0.0009765625	5.5697121003641e-05\\
0.00048828125	2.59133946812976e-05\\
0.000244140625	1.11308804955626e-05\\
0.0001220703125	3.72116963694925e-06\\
};
\addlegendentry{$c$ = 100};

\addplot [color=mycolor3,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.675756039940438\\
0.25	0.297226131944853\\
0.125	0.0825592844964573\\
0.0625	0.0208434937182301\\
0.03125	0.00525952318282813\\
0.015625	0.00151689927569931\\
0.0078125	0.000556943945510581\\
0.00390625	0.000245950322523599\\
0.001953125	0.000116625131437119\\
0.0009765625	5.57655913864862e-05\\
0.00048828125	2.59152410385158e-05\\
0.000244140625	1.10882670642735e-05\\
0.0001220703125	3.69347631910419e-06\\
};
\addlegendentry{$c$ = 1000};

\addplot [color=mycolor4,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.675756036781943\\
0.25	0.297226129034665\\
0.125	0.0825592875630795\\
0.0625	0.0208434885529682\\
0.03125	0.0052595182890019\\
0.015625	0.0015169010577403\\
0.0078125	0.000556946461668511\\
0.00390625	0.000245952362407769\\
0.001953125	0.000116625980033728\\
0.0009765625	5.57658747006021e-05\\
0.00048828125	2.59154612304772e-05\\
0.000244140625	1.10883344247597e-05\\
0.0001220703125	3.693476857833e-06\\
};
\addlegendentry{$c$ = 10000};


\addplot [color=black,dashed,line width=4.0pt]
  table[row sep=crcr]{%
0.5	0.5\\
0.25	0.25\\
0.125	0.125\\
0.0625	0.0625\\
0.03125	0.03125\\
0.015625	0.015625\\
0.0078125	0.0078125\\
0.00390625	0.00390625\\
0.001953125	0.001953125\\
0.0009765625	0.0009765625\\
0.00048828125	0.00048828125\\
0.000244140625	0.000244140625\\
0.0001220703125	0.0001220703125\\
6.103515625e-05	6.103515625e-05\\
3.0517578125e-05	3.0517578125e-05\\
};
\addlegendentry{$\mathcal{O}(\tau)$};

\end{axis}
\end{tikzpicture}%

==> figure12.tex <==
\definecolor{mycolor1}{rgb}{0.00000,0.00000,0.17241}%
\definecolor{mycolor2}{rgb}{1.00000,0.10345,0.72414}%
\definecolor{mycolor3}{rgb}{1.00000,0.82759,0.00000}%
\definecolor{mycolor4}{rgb}{0.00000,0.34483,0.00000}%
\definecolor{mycolor5}{rgb}{0.51724,0.51724,1.00000}%
\definecolor{mycolor6}{rgb}{0.62069,0.31034,0.27586}%
\definecolor{mycolor7}{rgb}{0.92900,0.69400,0.12500}%
%
\begin{tikzpicture}

\begin{axis}[%
width=2.0in,
height=2.5in,
at={(0.0in,0.0in)},
scale only axis,
xmode=log,
xmin=0.0001220703125,
xmax=0.5,
xminorticks=true,
xlabel style={font=\bfseries},
xlabel={$\tau$},
ymode=log,
ymin=1e-8,
ymax=0.9,
yminorticks=true,
xtick={1e-1, 1e-2, 1e-3, 1e-4},
ytick={1e-1, 1e-3, 1e-5, 1e-7, 1e-9},
ylabel style={font=\normalsize},
ylabel={$\text{Error in z}$},
axis background/.style={fill=white},
legend columns = 2,
legend style={yshift=-0.15cm,xshift=0.1cm,nodes={scale=0.6, transform shape},legend cell align=left,align=left,draw=white!10!black,legend pos=south east}
]
\addplot [color=blue,solid,line width=2.0pt,mark=triangle,mark options={solid}]
table[row sep=crcr]{%
0.5	0.055586532849719\\
0.25	0.0302184945538502\\
0.125	0.0114041066851084\\
0.0625	0.00549552730044718\\
0.03125	0.00291689193335499\\
0.015625	0.00152205228614517\\
0.0078125	0.00077736747890973\\
0.00390625	0.000390764257890963\\
0.001953125	0.000193588694460023\\
0.0009765625	9.39935830235904e-05\\
0.00048828125	4.39393287630912e-05\\
0.000244140625	1.88474182458886e-05\\
0.0001220703125	6.28519105127057e-06\\
};
\addlegendentry{ }; 

\addplot [color=blue,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.0899080256957936\\
0.25	0.0444683772178071\\
0.125	0.0134134660760305\\
0.0625	0.00352151149616598\\
0.03125	0.000896580640844523\\
0.015625	0.000226942467684025\\
0.0078125	5.82445133515841e-05\\
0.00390625	1.58237168341695e-05\\
0.001953125	4.98280075615585e-06\\
0.0009765625	2.18733555695913e-06\\
0.00048828125	9.86904485196557e-07\\
0.000244140625	4.18171590997296e-07\\
0.0001220703125	1.38814521572827e-07\\
};
\addlegendentry{$c$ = 1};

\addplot [color=green,solid,line width=2.0pt,mark=triangle,mark options={solid}]
table[row sep=crcr]{%
0.5	0.0405949868371809\\
0.25	0.0276991921488574\\
0.125	0.0145195529097185\\
0.0625	0.00749113351882388\\
0.03125	0.00644591290929173\\
0.015625	0.00286872912882958\\
0.0078125	0.00218644954628817\\
0.00390625	0.00126745389271027\\
0.001953125	0.000669986083834923\\
0.0009765625	0.000333382508532788\\
0.00048828125	0.000157636210380704\\
0.000244140625	6.79893846547049e-05\\
0.0001220703125	2.2734669135031e-05\\
};
\addlegendentry{ }; %10

\addplot [color=green,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.0301419535295789\\
0.25	0.012880759945936\\
0.125	0.00523172503120331\\
0.0625	0.00151069530428203\\
0.03125	0.000399838952689728\\
0.015625	0.00012343786511929\\
0.0078125	3.15951971898447e-05\\
0.00390625	8.23286187853966e-06\\
0.001953125	2.29378660782402e-06\\
0.0009765625	7.45261210685593e-07\\
0.00048828125	3.14664532413308e-07\\
0.000244140625	1.34240611712375e-07\\
0.0001220703125	4.46729218482998e-08\\
};
\addlegendentry{$c$ = 10};

\addplot [color=mycolor3,solid,line width=2.0pt,mark=triangle,mark options={solid}]
table[row sep=crcr]{%
0.5	0.057749585080492\\
0.25	0.0451347075134446\\
0.125	0.0244582643279609\\
0.0625	0.0118310846374097\\
0.03125	0.00567461033860597\\
0.015625	0.00275967336690062\\
0.0078125	0.001450914730349\\
0.00390625	0.000698001874463238\\
0.001953125	0.000343455478084603\\
0.0009765625	0.000219862594159145\\
0.00048828125	0.000123406541196853\\
0.000244140625	6.51725448382259e-05\\
0.0001220703125	1.322362114743e-05\\
};
\addlegendentry{ }; %100

\addplot [color=mycolor3,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.0335629622387554\\
0.25	0.0210046608107415\\
0.125	0.00640905315344857\\
0.0625	0.00179954954341054\\
0.03125	0.000462952193504262\\
0.015625	0.000128231402597365\\
0.0078125	3.26060501886914e-05\\
0.00390625	8.16209093678756e-06\\
0.001953125	2.06626707297798e-06\\
0.0009765625	6.41550456923502e-07\\
0.00048828125	2.44374972021419e-07\\
0.000244140625	9.41986317980642e-08\\
0.0001220703125	3.00764478287979e-08\\
};
\addlegendentry{$c$ = 100};

\addplot [color=red,solid,line width=2.0pt,mark=triangle,mark options={solid}]
table[row sep=crcr]{%
0.5	0.033886033399357\\
0.25	0.0377779299951301\\
0.125	0.0192799336222326\\
0.0625	0.0105138600915772\\
0.03125	0.00575092856179256\\
0.015625	0.00283440548298271\\
0.0078125	0.00140632374413447\\
0.00390625	0.000691883931390366\\
0.001953125	0.000343350909001317\\
0.0009765625	0.000165888814790438\\
0.00048828125	7.7514669997982e-05\\
0.000244140625	3.3335336366041e-05\\
0.0001220703125	1.11862572923234e-05\\
};
\addlegendentry{ }; %1000

\addplot [color=red,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.0338520284207542\\
0.25	0.0159280994236293\\
0.125	0.00613027331732125\\
0.0625	0.00162581175065432\\
0.03125	0.000462426839932938\\
0.015625	0.000125758071021153\\
0.0078125	3.21765173637443e-05\\
0.00390625	8.12006691080711e-06\\
0.001953125	2.10786291911464e-06\\
0.0009765625	6.4311493380261e-07\\
0.00048828125	2.45864578211815e-07\\
0.000244140625	9.45257879457367e-08\\
0.0001220703125	3.00487457060678e-08\\
};
\addlegendentry{$c$ = 1000};

\addplot [color=mycolor6,solid,line width=2.0pt,mark=triangle,mark options={solid}]
table[row sep=crcr]{%
0.5	0.0724476127627824\\
0.25	0.0430154566458451\\
0.125	0.0191428986032965\\
0.0625	0.00937051221102821\\
0.03125	0.00599191245102996\\
0.015625	0.00290944842299778\\
0.0078125	0.00142745312346152\\
0.00390625	0.000702581967810119\\
0.001953125	0.000344334021586022\\
0.0009765625	0.000166278934454716\\
0.00048828125	7.75150150765093e-05\\
0.000244140625	3.32185704347014e-05\\
0.0001220703125	1.10699041835372e-05\\
};
\addlegendentry{ };

\addplot [color=mycolor6,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.0345499968281657\\
0.25	0.0147240985635468\\
0.125	0.0061544337852569\\
0.0625	0.00187321007030227\\
0.03125	0.000479323407022923\\
0.015625	0.000130930072882889\\
0.0078125	3.30549739559009e-05\\
0.00390625	8.18354525953544e-06\\
0.001953125	2.06711176454066e-06\\
0.0009765625	6.42371250262216e-07\\
0.00048828125	2.45529769704581e-07\\
0.000244140625	9.45423832041964e-08\\
0.0001220703125	3.00336967890446e-08\\
};
\addlegendentry{$c$ = 10000};

\addlegendimage{empty legend}
\addlegendentry{ };

\addplot [color=black,dash dot,line width=4.0pt]
table[row sep=crcr]{%
	0.5	0.5\\
	0.25	0.25\\
	0.125	0.125\\
	0.0625	0.0625\\
	0.03125	0.03125\\
	0.015625	0.015625\\
	0.0078125	0.0078125\\
	0.00390625	0.00390625\\
	0.001953125	0.001953125\\
	0.0009765625	0.0009765625\\
	0.00048828125	0.00048828125\\
	0.000244140625	0.000244140625\\
	0.0001220703125	0.0001220703125\\
	6.103515625e-05	6.103515625e-05\\
	3.0517578125e-05	3.0517578125e-05\\
};
\addlegendentry{$\mathcal{O}(\tau)$};

\addlegendimage{empty legend}
\addlegendentry{ };

\addplot [color=black,dashed,line width=4.0pt]
table[row sep=crcr]{%
0.5	0.0125296808406818\\
0.25	0.00313242021017045\\
0.125	0.000783105052542613\\
0.0625	0.000195776263135653\\
0.03125	0.0000489440657839133\\
0.015625	0.0000122360164459783\\
0.0078125	0.00000305900411149458\\
0.00390625	7.64751027873645e-07\\
0.001953125	1.91187756968411e-07\\
0.0009765625	4.77969392421028e-08\\
0.00048828125	1.19492348105257e-08\\
0.000244140625	2.98730870263143e-09\\
0.0001220703125	7.46827175657857e-10\\
6.103515625e-05	1.86706793914464e-10\\
3.0517578125e-05	4.6676698478616e-11\\
};
\addlegendentry{$\mathcal{O}(\tau^2)$};

\end{axis}

\begin{axis}[%
width=2.0in,
height=2.5in,
at={(3.0in,0.0in)},
scale only axis,
xmode=log,
xmin=0.0001220703125,
xmax=0.5,
xminorticks=true,
xlabel style={font=\bfseries},
xlabel={$\tau$},
ymode=log,
ymin=1e-8,
ymax=0.9,
yminorticks=true,
xtick={1e-1, 1e-2, 1e-3, 1e-4},
ytick={1e-1, 1e-3, 1e-5, 1e-7, 1e-9},
ylabel style={font=\normalsize},
ylabel={$\text{Error in n}$},
axis background/.style={fill=white},
legend columns = 2,
legend style={yshift=-0.15cm,xshift=0.1cm,nodes={scale=0.6, transform shape},legend cell align=left,align=left,draw=white!10!black,legend pos=south east},
]
\addplot [color=blue,solid,line width=2.0pt,mark=triangle,mark options={solid}]
table[row sep=crcr]{%
0.5	0.676486292235307\\
0.25	0.297250067157146\\
0.125	0.0838030102284134\\
0.0625	0.0221634410753464\\
0.03125	0.00607799576009037\\
0.015625	0.00180226425110685\\
0.0078125	0.000628766074286798\\
0.00390625	0.000259820097101336\\
0.001953125	0.000118251956673363\\
0.0009765625	5.54046878194233e-05\\
0.00048828125	2.54984309292628e-05\\
0.000244140625	1.08588123716483e-05\\
0.0001220703125	3.60872225568945e-06\\
};
\addlegendentry{ }; %1

\addplot [color=blue,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.676505037295983\\
0.25	0.297528854856633\\
0.125	0.0834360032171618\\
0.0625	0.021366427773956\\
0.03125	0.00540455774717528\\
0.015625	0.00134600425816962\\
0.0078125	0.000334624616174413\\
0.00390625	8.33575821463699e-05\\
0.001953125	2.07896993923461e-05\\
0.0009765625	5.1799028366964e-06\\
0.00048828125	1.28087346197441e-06\\
0.000244140625	3.05991611665001e-07\\
0.0001220703125	6.17007640963188e-08\\
};
\addlegendentry{$c$ = 1};

\addplot [color=green,solid,line width=2.0pt,mark=triangle,mark options={solid}]
table[row sep=crcr]{%
0.5	0.675727109539905\\
0.25	0.297102189953057\\
0.125	0.0823252573502638\\
0.0625	0.0206792674447262\\
0.03125	0.00506701668564554\\
0.015625	0.0014411828559432\\
0.0078125	0.000523160654445462\\
0.00390625	0.000234051122308833\\
0.001953125	0.000111733198731171\\
0.0009765625	5.35615879389074e-05\\
0.00048828125	2.49136441282593e-05\\
0.000244140625	1.06635388056017e-05\\
0.0001220703125	3.55253656157172e-06\\
};
\addlegendentry{ }; %10

\addplot [color=green,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.675721918976389\\
0.25	0.29729315974358\\
0.125	0.0817710951950862\\
0.0625	0.0202566763926082\\
0.03125	0.00494489520124711\\
0.015625	0.00121730002794884\\
0.0078125	0.00030150240934686\\
0.00390625	7.50290243644981e-05\\
0.001953125	1.87042723318379e-05\\
0.0009765625	4.65772421095722e-06\\
0.00048828125	1.15022704742334e-06\\
0.000244140625	2.73832663806725e-07\\
0.0001220703125	5.47743203296122e-08\\
};
\addlegendentry{$c$ = 10};

\addplot [color=mycolor3,solid,line width=2.0pt,mark=triangle,mark options={solid}]
table[row sep=crcr]{%
0.5	0.675755913057\\
0.25	0.297224369103591\\
0.125	0.0825582419832529\\
0.0625	0.0208445960414273\\
0.03125	0.00525945405303095\\
0.015625	0.00151638558077684\\
0.0078125	0.000556521393103677\\
0.00390625	0.00024566425292134\\
0.001953125	0.000116480987311607\\
0.0009765625	5.5697121003641e-05\\
0.00048828125	2.59133946812976e-05\\
0.000244140625	1.11308804955626e-05\\
0.0001220703125	3.72116963694925e-06\\
};
\addlegendentry{ }; %100

\addplot [color=mycolor3,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.675750148592486\\
0.25	0.297361122733621\\
0.125	0.0817941350579321\\
0.0625	0.0202448566383005\\
0.03125	0.00493994451181839\\
0.015625	0.00121692650493198\\
0.0078125	0.000301992094557656\\
0.00390625	7.52054427608836e-05\\
0.001953125	1.8753264546937e-05\\
0.0009765625	4.67072086468778e-06\\
0.00048828125	1.15350272988105e-06\\
0.000244140625	2.74778308273805e-07\\
0.0001220703125	5.48737784066105e-08\\
};
\addlegendentry{$c$ = 100};

\addplot [color=red,solid,line width=2.0pt,mark=triangle,mark options={solid}]
table[row sep=crcr]{%
0.5	0.675756039940438\\
0.25	0.297226131944853\\
0.125	0.0825592844964573\\
0.0625	0.0208434937182301\\
0.03125	0.00525952318282813\\
0.015625	0.00151689927569931\\
0.0078125	0.000556943945510581\\
0.00390625	0.000245950322523599\\
0.001953125	0.000116625131437119\\
0.0009765625	5.57655913864862e-05\\
0.00048828125	2.59152410385158e-05\\
0.000244140625	1.10882670642735e-05\\
0.0001220703125	3.69347631910419e-06\\
};
\addlegendentry{ }; %1.000

\addplot [color=red,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.675750386258943\\
0.25	0.297362052366988\\
0.125	0.081794189127449\\
0.0625	0.020244471350598\\
0.03125	0.00493984110767467\\
0.015625	0.00121691739549571\\
0.0078125	0.000301990265316989\\
0.00390625	7.52044494496727e-05\\
0.001953125	1.87525419610355e-05\\
0.0009765625	4.67017683958848e-06\\
0.00048828125	1.15335690457993e-06\\
0.000244140625	2.74587418065081e-07\\
0.0001220703125	5.49269158371682e-08\\
};
\addlegendentry{$c$ = 1000};

\addplot [color=mycolor6,solid,line width=2.0pt,mark=triangle,mark options={solid}]
table[row sep=crcr]{%
0.5	0.675756036781943\\
0.25	0.297226129034665\\
0.125	0.0825592875630795\\
0.0625	0.0208434885529682\\
0.03125	0.0052595182890019\\
0.015625	0.0015169010577403\\
0.0078125	0.000556946461668511\\
0.00390625	0.000245952362407769\\
0.001953125	0.000116625980033728\\
0.0009765625	5.57658747006021e-05\\
0.00048828125	2.59154612304772e-05\\
0.000244140625	1.10883344247597e-05\\
0.0001220703125	3.693476857833e-06\\
};
\addlegendentry{ }; %10.000

\addplot [color=mycolor6,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.675750388640031\\
0.25	0.297362058884099\\
0.125	0.0817941906717678\\
0.0625	0.0202444680563113\\
0.03125	0.00493984005597546\\
0.015625	0.00121691730898388\\
0.0078125	0.000301990250324558\\
0.00390625	7.52044390371479e-05\\
0.001953125	1.87525352987168e-05\\
0.0009765625	4.67017337743347e-06\\
0.00048828125	1.15335513820948e-06\\
0.000244140625	2.74586599664161e-07\\
0.0001220703125	5.49266403608985e-08\\
};
\addlegendentry{$c$ = 10000};

\addlegendimage{empty legend}
\addlegendentry{ };

\addplot [color=black,dash dot,line width=4.0pt]
table[row sep=crcr]{%
	0.5	0.5\\
	0.25	0.25\\
	0.125	0.125\\
	0.0625	0.0625\\
	0.03125	0.03125\\
	0.015625	0.015625\\
	0.0078125	0.0078125\\
	0.00390625	0.00390625\\
	0.001953125	0.001953125\\
	0.0009765625	0.0009765625\\
	0.00048828125	0.00048828125\\
	0.000244140625	0.000244140625\\
	0.0001220703125	0.0001220703125\\
	6.103515625e-05	6.103515625e-05\\
	3.0517578125e-05	3.0517578125e-05\\
};
\addlegendentry{$\mathcal{O}(\tau)$};

\addlegendimage{empty legend}
\addlegendentry{ };

\addplot [color=black,dashed,line width=4.0pt]
table[row sep=crcr]{%
0.5	0.125296808406818\\
0.25	0.0313242021017045\\
0.125	0.00783105052542613\\
0.0625	0.00195776263135653\\
0.03125	0.000489440657839133\\
0.015625	0.000122360164459783\\
0.0078125	0.0000305900411149458\\
0.00390625	7.64751027873645e-06\\
0.001953125	1.91187756968411e-06\\
0.0009765625	4.77969392421028e-07\\
0.00048828125	1.19492348105257e-07\\
0.000244140625	2.98730870263143e-08\\
0.0001220703125	7.46827175657857e-09\\
6.103515625e-05	1.86706793914464e-09\\
3.0517578125e-05	4.6676698478616e-10\\
};
\addlegendentry{$\mathcal{O}(\tau^2)$};

\end{axis}
\end{tikzpicture}%

==> figure2.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.00000,0.17241}%
\definecolor{mycolor2}{rgb}{1.00000,0.10345,0.72414}%
\definecolor{mycolor3}{rgb}{1.00000,0.82759,0.00000}%
\definecolor{mycolor4}{rgb}{0.00000,0.34483,0.00000}%
\definecolor{mycolor5}{rgb}{0.51724,0.51724,1.00000}%
\definecolor{mycolor6}{rgb}{0.62069,0.31034,0.27586}%
\definecolor{mycolor7}{rgb}{0.92900,0.69400,0.12500}%
%
\begin{tikzpicture}

\begin{axis}[%
width=2.0in,
height=2.5in,
at={(0.0in,0.0in)},
scale only axis,
xmode=log,
xmin=0.0001220703125,
xmax=0.5,
xminorticks=true,
xlabel style={font=\bfseries},
xlabel={$\tau$},
ymode=log,
ymin=1e-8,
ymax=0.9,
yminorticks=true,
xtick={1e-1, 1e-2, 1e-3, 1e-4},
ytick={1e-1, 1e-3, 1e-5, 1e-7, 1e-8},
ylabel style={font=\normalsize},
ylabel={$\text{Error in z}$},
axis background/.style={fill=white},
legend style={yshift=-0.15cm,xshift=0.1cm,nodes={scale=0.7, transform shape},legend cell align=left,align=left,draw=white!10!black,legend pos=south east}
]
\addplot [color=blue,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.0899080256957936\\
0.25	0.0444683772178071\\
0.125	0.0134134660760305\\
0.0625	0.00352151149616598\\
0.03125	0.000896580640844523\\
0.015625	0.000226942467684025\\
0.0078125	5.82445133515841e-05\\
0.00390625	1.58237168341695e-05\\
0.001953125	4.98280075615585e-06\\
0.0009765625	2.18733555695913e-06\\
0.00048828125	9.86904485196557e-07\\
0.000244140625	4.18171590997296e-07\\
0.0001220703125	1.38814521572827e-07\\
};
\addlegendentry{$c$ = 1};

\addplot [color=red,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.0301419535295789\\
0.25	0.012880759945936\\
0.125	0.00523172503120331\\
0.0625	0.00151069530428203\\
0.03125	0.000399838952689728\\
0.015625	0.00012343786511929\\
0.0078125	3.15951971898447e-05\\
0.00390625	8.23286187853966e-06\\
0.001953125	2.29378660782402e-06\\
0.0009765625	7.45261210685593e-07\\
0.00048828125	3.14664532413308e-07\\
0.000244140625	1.34240611712375e-07\\
0.0001220703125	4.46729218482998e-08\\
};
\addlegendentry{$c$ = 10};

\addplot [color=green,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.0335629622387554\\
0.25	0.0210046608107415\\
0.125	0.00640905315344857\\
0.0625	0.00179954954341054\\
0.03125	0.000462952193504262\\
0.015625	0.000128231402597365\\
0.0078125	3.26060501886914e-05\\
0.00390625	8.16209093678756e-06\\
0.001953125	2.06626707297798e-06\\
0.0009765625	6.41550456923502e-07\\
0.00048828125	2.44374972021419e-07\\
0.000244140625	9.41986317980642e-08\\
0.0001220703125	3.00764478287979e-08\\
};
\addlegendentry{$c$ = 100};

\addplot [color=mycolor3,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.0338520284207542\\
0.25	0.0159280994236293\\
0.125	0.00613027331732125\\
0.0625	0.00162581175065432\\
0.03125	0.000462426839932938\\
0.015625	0.000125758071021153\\
0.0078125	3.21765173637443e-05\\
0.00390625	8.12006691080711e-06\\
0.001953125	2.10786291911464e-06\\
0.0009765625	6.4311493380261e-07\\
0.00048828125	2.45864578211815e-07\\
0.000244140625	9.45257879457367e-08\\
0.0001220703125	3.00487457060678e-08\\
};
\addlegendentry{$c$ = 1000};

\addplot [color=mycolor4,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.0345499968281657\\
0.25	0.0147240985635468\\
0.125	0.0061544337852569\\
0.0625	0.00187321007030227\\
0.03125	0.000479323407022923\\
0.015625	0.000130930072882889\\
0.0078125	3.30549739559009e-05\\
0.00390625	8.18354525953544e-06\\
0.001953125	2.06711176454066e-06\\
0.0009765625	6.42371250262216e-07\\
0.00048828125	2.45529769704581e-07\\
0.000244140625	9.45423832041964e-08\\
0.0001220703125	3.00336967890446e-08\\
};
\addlegendentry{$c$ = 10000};

\addplot [color=black,dashed,line width=4.0pt]
table[row sep=crcr]{%
0.5	0.0125296808406818\\
0.25	0.00313242021017045\\
0.125	0.000783105052542613\\
0.0625	0.000195776263135653\\
0.03125	0.0000489440657839133\\
0.015625	0.0000122360164459783\\
0.0078125	0.00000305900411149458\\
0.00390625	7.64751027873645e-07\\
0.001953125	1.91187756968411e-07\\
0.0009765625	4.77969392421028e-08\\
0.00048828125	1.19492348105257e-08\\
0.000244140625	2.98730870263143e-09\\
0.0001220703125	7.46827175657857e-10\\
6.103515625e-05	1.86706793914464e-10\\
3.0517578125e-05	4.6676698478616e-11\\
};
\addlegendentry{$\mathcal{O}(\tau^2)$};

\end{axis}

\begin{axis}[%
width=2.0in,
height=2.5in,
at={(3.0in,0.0in)},
scale only axis,
xmode=log,
xmin=0.0001220703125,
xmax=0.5,
xminorticks=true,
xlabel style={font=\bfseries},
xlabel={$\tau$},
ymode=log,
ymin=1e-8,
ymax=0.9,
yminorticks=true,
xtick={1e-1, 1e-2, 1e-3, 1e-4},
ytick={1e-1, 1e-3, 1e-5, 1e-7, 1e-8},
ylabel style={font=\normalsize},
ylabel={$\text{Error in n}$},
axis background/.style={fill=white},
legend style={yshift=-0.15cm,xshift=0.1cm,nodes={scale=0.7, transform shape},legend cell align=left,align=left,draw=white!10!black,legend pos=south east}
]
\addplot [color=blue,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.676505037295983\\
0.25	0.297528854856633\\
0.125	0.0834360032171618\\
0.0625	0.021366427773956\\
0.03125	0.00540455774717528\\
0.015625	0.00134600425816962\\
0.0078125	0.000334624616174413\\
0.00390625	8.33575821463699e-05\\
0.001953125	2.07896993923461e-05\\
0.0009765625	5.1799028366964e-06\\
0.00048828125	1.28087346197441e-06\\
0.000244140625	3.05991611665001e-07\\
0.0001220703125	6.17007640963188e-08\\
};
\addlegendentry{$c$ = 1};

\addplot [color=red,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.675721918976389\\
0.25	0.29729315974358\\
0.125	0.0817710951950862\\
0.0625	0.0202566763926082\\
0.03125	0.00494489520124711\\
0.015625	0.00121730002794884\\
0.0078125	0.00030150240934686\\
0.00390625	7.50290243644981e-05\\
0.001953125	1.87042723318379e-05\\
0.0009765625	4.65772421095722e-06\\
0.00048828125	1.15022704742334e-06\\
0.000244140625	2.73832663806725e-07\\
0.0001220703125	5.47743203296122e-08\\
};
\addlegendentry{$c$ = 10};

\addplot [color=green,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.675750148592486\\
0.25	0.297361122733621\\
0.125	0.0817941350579321\\
0.0625	0.0202448566383005\\
0.03125	0.00493994451181839\\
0.015625	0.00121692650493198\\
0.0078125	0.000301992094557656\\
0.00390625	7.52054427608836e-05\\
0.001953125	1.8753264546937e-05\\
0.0009765625	4.67072086468778e-06\\
0.00048828125	1.15350272988105e-06\\
0.000244140625	2.74778308273805e-07\\
0.0001220703125	5.48737784066105e-08\\
};
\addlegendentry{$c$ = 100};

\addplot [color=mycolor3,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.675750386258943\\
0.25	0.297362052366988\\
0.125	0.081794189127449\\
0.0625	0.020244471350598\\
0.03125	0.00493984110767467\\
0.015625	0.00121691739549571\\
0.0078125	0.000301990265316989\\
0.00390625	7.52044494496727e-05\\
0.001953125	1.87525419610355e-05\\
0.0009765625	4.67017683958848e-06\\
0.00048828125	1.15335690457993e-06\\
0.000244140625	2.74587418065081e-07\\
0.0001220703125	5.49269158371682e-08\\
};
\addlegendentry{$c$ = 1000};

\addplot [color=mycolor4,solid,line width=2.0pt,mark=o,mark options={solid}]
table[row sep=crcr]{%
0.5	0.675750388640031\\
0.25	0.297362058884099\\
0.125	0.0817941906717678\\
0.0625	0.0202444680563113\\
0.03125	0.00493984005597546\\
0.015625	0.00121691730898388\\
0.0078125	0.000301990250324558\\
0.00390625	7.52044390371479e-05\\
0.001953125	1.87525352987168e-05\\
0.0009765625	4.67017337743347e-06\\
0.00048828125	1.15335513820948e-06\\
0.000244140625	2.74586599664161e-07\\
0.0001220703125	5.49266403608985e-08\\
};
\addlegendentry{$c$ = 10000};

\addplot [color=black,dashed,line width=4.0pt]
table[row sep=crcr]{%
0.5	0.125296808406818\\
0.25	0.0313242021017045\\
0.125	0.00783105052542613\\
0.0625	0.00195776263135653\\
0.03125	0.000489440657839133\\
0.015625	0.000122360164459783\\
0.0078125	0.0000305900411149458\\
0.00390625	7.64751027873645e-06\\
0.001953125	1.91187756968411e-06\\
0.0009765625	4.77969392421028e-07\\
0.00048828125	1.19492348105257e-07\\
0.000244140625	2.98730870263143e-08\\
0.0001220703125	7.46827175657857e-09\\
6.103515625e-05	1.86706793914464e-09\\
3.0517578125e-05	4.6676698478616e-10\\
};
\addlegendentry{$\mathcal{O}(\tau^2)$};

\end{axis}
\end{tikzpicture}%
